VM-NeRF: Tackling Sparsity in NeRF with View Morphing

NeRF aims to learn a continuous neural scene representation by using a finite set of input images taken from various viewpoints. A well-known limitation of NeRF methods is their reliance on data: the fewer the viewpoints, the higher the likelihood of overfitting. This paper addresses this issue by introducing a novel method to generate geometrically consistent image transitions between viewpoints using View Morphing. Our VM-NeRF approach requires no prior knowledge about the scene structure, as View Morphing is based on the fundamental principles of projective geometry. VM-NeRF tightly integrates this geometric view generation process during the training procedure of standard NeRF approaches. Notably, our method significantly improves novel view synthesis, particularly when only a few views are available. Experimental evaluation reveals consistent improvement over current methods that handle sparse viewpoints in NeRF models. We report an increase in PSNR of up to 1.8dB and 1.0dB when training uses eight and four views, respectively. Source code: \url{https://github.com/mbortolon97/VM-NeRF}

==> sections/impact_discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Potential impact of VM-NeRF on the society}
\label{sec:social_impact}
% Improvements in the task of few-viewpoints NVS, such as VM-NeRF, can be beneficial in many scenarios where it is not possible or feasible to acquire many images of the subjects.
% At the same time, these improvements can also facilitate the acquisition of a subject without their consent \cite{niemeyer2021regnerf}.
% This risk can be mitigated using cryptographic technologies that track if the input images was acquired with the subject permission and report it in the resulting NVS~\cite{sun2005robust}.

VM-NeRF requires the availability of specialised AI processors, such as GPUs, that can be expensive to access.
The per-scene optimisation procedure limits dataset-bias problems, improving fairness but requires more computation power, increasing the GPUs availability problem.
GPUs usage also has an environmental impact thanks to its high energy requirements.
The appearance of architectures that require considerably less computational time and, consequently, energy to optimise the scene can reduce this problem but present a novel set of challenges that need to be addressed.
We will explore this direction as a future work.

==> tables/psnr.tex <==
\begin{table*}[t]
\centering
\caption{PSNR metric per-scene results on the NeRF realistic synthetic 360$^\circ$ dataset.}
\label{tab:psnr_per_scene}
\resizebox{\textwidth}{!}{
\begin{tabular}{clccccccccc}
\toprule
\# views &                                                   Method & Chair & Drums & Ficus & Hot Dog & Lego & Materials &   Mic & Ship & \textbf{Avg} \\
\midrule
\textit{100} & \textit{NeRF \cite{mildenhall2020nerf}} & 34.57 & 25.71 & 29.05 & 36.88 & 31.47 & 29.49 & 33.05 & 29.48 & \textit{31.21} \\
\midrule
\multirow{2}{*}{8} & NeRF \cite{mildenhall2020nerf} w/ oracle images & 29.91 & 21.65 & 21.98 & 31.42 & 26.72 & 23.35 & 28.95 & 25.14 & \textit{26.14} \\
 & VM-NeRF w/ oracle depth & 28.39 & 21.13 & 21.95 & 27.05 & 23.76 & 21.12 & 27.00 & 23.37 & \textit{24.22} \\
\midrule
\multirow{5}{*}{8} & NeRF \cite{mildenhall2020nerf} & 25.11 & 19.93 & \textbf{21.72} & 23.19 & 24.65 & 21.95 & 27.81 & 23.27  & \textit{23.45} \\
 & DietNeRF \cite{jain2021dietnerf} & 26.01 & 18.79 & 20.89 & 26.01 & 21.55 & 21.28 & 27.32 & 21.99 & \textit{22.98} \\
 & AugNeRF \cite{chen2022augnerf} & 15.05 & 0.75 & 14.86 & 12.50 & 1.04 & 9.94 & 13.40 & 12.81 & \textit{10.04} \\
 & RegNeRF \cite{niemeyer2021regnerf} & 23.12 & 16.13 & 20.88 & 26.81 & 24.33 & 21.11 & \textbf{28.22} & 22.72 & \textit{22.91} \\
 & VM-NeRF (ours) & \textbf{27.87} & \textbf{20.20} & 21.36 & 27.15 & \textbf{24.84} & \textbf{22.35} & 27.61 & \textbf{23.71} & \textbf{\textit{24.39}} \\
\midrule
\multirow{4}{*}{8 \cite{jain2021dietnerf}} & NeRF \cite{mildenhall2020nerf} & 25.11 & 19.93 & \textbf{21.72} & 23.19 & 24.65 & 21.95 & \textbf{27.81} & 23.27 & \textit{20.09} \\
 & DietNeRF \cite{jain2021dietnerf} & 26.01 & 18.79 & 20.89 & 26.01 & 21.55 & 21.28 & 27.32 & 21.99 & \textit{23.59} \\
 & VM-NeRF (ours) & \textbf{26.90} & \textbf{20.03} & 20.46 & \textbf{29.08} & \textbf{24.79} & \textbf{21.98} & 26.39 & \textbf{23.50} & \textbf{\textit{24.14}} \\
\midrule
\multirow{5}{*}{4} & NeRF \cite{mildenhall2020nerf} & 14.11 & 10.45 & 14.29 & 10.35 & 9.38 & 8.28 & 13.13 & 7.85 & \textit{10.98} \\
 & DietNeRF \cite{jain2021dietnerf} & 19.88 & 9.84 & 17.77 & 9.99 & 8.97 & 16.43 & 11.04 & 6.94 & \textit{12.61} \\
 & AugNeRF \cite{chen2022augnerf} & 13.57 & 11.18 & 14.16 & 1.05 & 9.82 & 1.12 & 11.94 & 2.27 & \textit{8.14} \\
 & RegNeRF \cite{niemeyer2021regnerf} & 15.45 & 11.88 & 14.78 & \textbf{15.64} & 12.50 & 16.37 & \textbf{24.48} & \textbf{15.91} & \textit{15.88} \\
 & VM-NeRF (ours) & \textbf{22.49} & \textbf{16.71} & \textbf{18.68} & 10.84 & \textbf{19.86} & \textbf{18.72} & 20.79 & 7.15 & \textbf{\textit{16.90}} \\
\bottomrule
\end{tabular}
}
\end{table*}
